Semantic Word Clusters Using Signed Normalized Graph Cuts

Vector space representations of words capture many aspects of word similarity, but such methods tend to make vector spaces in which antonyms (as well as synonyms) are close to each other. We present a new signed spectral normalized graph cut algorithm, signed clustering, that overlays existing thesauri upon distributionally derived vector representations of words, so that antonym relationships between word pairs are represented by negative weights. Our signed clustering algorithm produces clusters of words which simultaneously capture distributional and synonym relations. We evaluate these clusters against the SimLex-999 dataset (Hill et al.,2014) of human judgments of word pair similarities, and also show the benefit of using our clusters to predict the sentiment of a given text.

==> sections/theory_abridged.tex <==
\section{Signed Graph Cluster Estimation}

\subsection{Signed Normalized Cut}

Signed graphs allow negative and positive entries in a symmetric matrix (the weight matrix $W$).
Such graphs (with weights $(-1, 0, +1)$) were introduced as early as
1953 by  \cite{harary1953notion}, to model social relations involving disliking,
indifference, and liking.  The problem of clustering the nodes
of a signed graph arises naturally as a generalization of the
clustering problem for weighted graphs. Figure 1 shows a signed graph of word similarities with a thesaurus overlay.
\begin{figure}[ht]
  \label{fig:dc2}
   \includegraphics[width=\linewidth]{signed_word_cluster.jpg}
  \caption{Signed graph of words using 
  the heat kernel of the Euclidean distance from the word embedding. The red edges represent the antonym relation while blue edges represent synonymy relations.}
\end{figure}
%We extend normalized cuts signed graphs in order to incorporate antonym information into word clusters.

\theoremstyle{definition}
\begin{definition}
\label{graph-weighted}
A {\it  weighted graph\/} 
is a pair $G = (V, W)$, where 
$V = \{v_1,  \ldots, v_m\}$ is a set of
{\it nodes\/} or {\it vertices\/}, and $W$ is a symmetric matrix
called the {\it weight matrix\/}, such that $w_{i\, j} \geq 0$
for all $i, j \in \{1, \ldots, m\}$, 
and $w_{i\, i} = 0$ for $i = 1, \ldots, m$.
We say that a set $\{v_i, v_j\}$  is an edge iff
$w_{i\, j} > 0$. The corresponding (undirected) graph $(V, E)$
with $E = \{\{v_i, v_j\} \mid w_{i\, j} > 0\}$, 
is called the {\it underlying graph\/} of $G$.
\end{definition}

Given a signed graph $G = (V, W)$ (where $W$ is a symmetric matrix
with zero diagonal entries), the {\it underlying graph\/} of $G$ is
the graph with node set $V$ and set of (undirected) edges
$E = \{\{v_i, v_j\} \mid w_{i j} \not= 0\}$.

If $(V, W)$ is a signed graph, where $W$ is an $m\times m$ symmetric
matrix with zero diagonal entries and with the other entries
$w_{i j}\in \reals$ arbitrary, for any node $v_i \in V$, the {\it signed degree\/} of $v_i$ is defined as
\[
\overline{d}_i = \overline{d}(v_i) = \sum_{j = 1}^m |w_{i j}|,
\]
and the {\it signed degree matrix \/} $\overline{\Degsym}$ as
\[
\overline{\Degsym} = \mathrm{diag}(\overline{d}(v_1) , \ldots, \overline{d}(v_m)).
\]
For any subset $A$ of the set of nodes
$V$, let
\[
\mathrm{vol}(A) = \sum_{v_i\in A} \overline{d}_i = 
 \sum_{v_i\in A} \sum_{j = 1}^m |w_{i j}|.
\]
For any two subsets $A$ and $B$ of $V$, 
define $\mathrm{links}^+(A,B)$, 
$\mathrm{links}^-(A,B)$, and $\mathrm{cut}(A,\overline{A})$ by
\begin{align*}
\mathrm{links}^+(A, B)  = 
\sum_{\begin{subarray}{c}
v_i \in A, v_j\in B \\
w_{i j} > 0
\end{subarray}
} 
w_{i j} \\
%\text{ \ \  \ \ \   } 
\mathrm{links}^-(A,B)  = 
\sum_{\begin{subarray}{c}
v_i \in A, v_j\in B \\
w_{i j} < 0
\end{subarray}
}
- w_{i j} \\
\mathrm{cut}(A,\overline{A})  = 
\sum_{\begin{subarray}{c}
v_i \in A, v_j\in \overline{A} \\
w_{i j} \not=  0
\end{subarray}
}
|w_{i j}| .
\end{align*}
%Note that
%$\mathrm{links}^+(A, B) = \mathrm{links}^+(B, A)$,  $\mathrm{links}^-(A,
%B) = \mathrm{links}^-(B, A)$,  and 
%\[
%\mathrm{cut}(A,\overline{A})  =  \mathrm{links}^+(A,\overline{A}) + \mathrm{links}^-(A,\overline{A}) .
%\]
Then, the {\it signed Laplacian\/} $\overline{L}$ is defined by
\[
\overline{L} = \overline{\Degsym} - W, 
\]
and its normalized version $\overline{L}_{\mathrm{sym}}$ by
\[
\overline{L}_{\mathrm{sym}} =  \overline{\Degsym}^{-1/2}\, \overline{L}\,
\overline{\Degsym}^{-1/2}
= I - \overline{\Degsym}^{-1/2} W \overline{\Degsym}^{-1/2}.  
\]
For a graph without isolated vertices, we have $\overline{d}(v_i) > 0$
for $i = 1, \ldots, m$, so $\overline{\Degsym}^{-1/2}$ is well defined.

\begin{proposition}
\label{Laplace1s}
For any  $m\times m$ symmetric matrix $W = (w_{i j})$, if we let $\overline{L} = \overline{\Degsym} - W$
where $\overline{\Degsym}$ is the signed degree matrix associated with $W$,
then  we have
\[
\transpos{x} \overline{L} x =
\frac{1}{2}\sum_{i, j = 1}^m |w_{i  j}| (x_i - \mathrm{sgn}(w_{i j}) x_j)^2
\quad\mathrm{for\ all}\> x\in \reals^m.
\]
Consequently, $\overline{L}$  is positive semidefinite.
\end{proposition}

Given a partition of $V$ into $K$
clusters $(A_1, \ldots, A_K)$, if we represent the $j$th block of
this partition by a vector $X^j$ such that
\[
X^j_i = 
\begin{cases}
a_j & \text{if $v_i \in A_j$} \\
0 &  \text{if $v_i \notin A_j$} ,
\end{cases}
\]
for some $a_j \not= 0$.

\begin{definition}
\label{sncut}
The {\it signed normalized cut\/}
$\mathrm{sNcut}(A_1, \ldots, A_K)$ of the
partition $(A_1, \ldots, A_K)$ is defined as

\[
\mathrm{sNcut}(A_1, \ldots, A_K) = 
\sum_{j = 1}^K \frac{\transpos{(X^j)} \overline{L} X^j} 
  {\transpos{(X^j)} \overline{\Degsym} X^j}.
\]
where $X$ is the $N\times K$ matrix whose $j$th column is $X^j$.
\end{definition}

Minimizing $\mathrm{sNcut}(A_1, \ldots, A_K)$ amounts to 
minimizing the number of positive between clusters,
and also minimizing the number of negative edges within clusters.

\subsection{Optimization Problem}


We have our first formulation of $K$-way clustering
of a graph using normalized cuts, called problem PNC1:

If we let
\begin{align*}
\s{X}  = \Big\{[X^1\> \ldots \> X^K] \mid
X^j = a_j(x_1^j, \ldots, x_N^j) , \\
\>
x_i^j \in \{1, 0\},
 a_j\in \reals, \> X^j \not= 0
\Big\}
\end{align*}

our solution set is
\[
\s{K}  = \big\{
X  \in\s{X}  \mid \transpos{X}  \overline{\Degsym}\mathbf{1} = 0
\big\}.
\]

\medskip\noindent
{\bf $K$-way Clustering of a graph using Normalized Cut, Version 1: \\
Problem PNC1}


\begin{align*}
& \mathrm{minimize}     &  \sum_{j = 1}^K 
\frac{\transpos{(X^j)} \overline{L} X^j}{\transpos{(X^j)}\overline{\Degsym} X^j}& &  &  &\\
& \mathrm{subject\ to} & 
 \transpos{(X^i)} \overline{\Degsym} X^j = 0,  & &  &  &\\
& & \quad 1\leq i, j \leq K,\> 
i\not= j,  & &  X\in \s{X}. & &  & 
\end{align*}


%An equivalent version of the optimization problem is

%\medskip\noindent


%{\bf Problem PNC2}
%
%\begin{align*}
%& \mathrm{minimize}     &  &  
%\mathrm{tr}(\transpos{X} \overline{L} X)& &  &  &\\
%& \mathrm{subject\ to} &  & 
%\transpos{X} \overline{\Degsym} X = I, 
% & &  X\in \s{X}. & &
%\end{align*}


We obtain the relaxed problem by the unconstrained the solution without $X\in \s{X}$


\medskip\noindent
{\bf Problem $(*_2)$}

\begin{align*}
& \mathrm{minimize}     &  &  
\mathrm{tr}(\transpos{Y}\overline{\Degsym}^{-1/2} \overline{L} \overline{\Degsym}^{-1/2} Y)& &  &  &\\
& \mathrm{subject\ to} &  & 
\transpos{Y} Y = I. 
 & &  & &  
\end{align*}

The minimum of  problem $(*_2)$
is achieved by any $K$ unit eigenvectors $(u_1, \ldots, u_K)$ associated with the smallest
eigenvalues
\[
0 \leq \nu_1\leq  \nu_2 \leq  \ldots \leq  \nu_K
\]
of $L_{\mathrm{sym}}$.

\subsection{Finding an Approximate Discrete Solution}

Given a solution $Z$ of problem $(*_2)$, 
we  look for pairs
$(X, Q)$ with $X\in \s{X}$ and  where $Q$ is a $K\times K$ matrix with
nonzero and pairwise orthogonal columns,
with $\norme{X}_F = \norme{Z}_F$,
that minimize
\[
\varphi(X, Q) = \norme{X - ZQ}_F.
\]
Here, $\norme{A}_F$ is the Frobenius norm of $A$.

This is a challenging nonlinear optimization problem.
To simplify the problem, we proceed by alternating steps during which we minimize 
$\varphi(X, Q)$ with respect to $X$ holding $Q$ fixed, and vice versa.
This second step in which $X$ is held fixed has no known closed--form solution, thus we simplify the problem.
We minimize $\norme{X - ZR\Lambda}_F$ in two stages.
In stage 1, the problem reduces to  maximizing   $\mathrm{tr}(\transpos{Q}\transpos{Z}X)$.

\begin{enumerate}
\item
We set $\Lambda = I$ and find $R\in \mathbf{O}(K)$
that minimizes  $\norme{X - ZR}_F$.
\item
Given $X$, $Z$, and $R$,  find a 
diagonal invertible matrix $\Lambda$ that
minimizes  $\norme{X - ZR\Lambda}_F$.
\end{enumerate}

%The matrix $R\Lambda$ is not a minimizer of
%$\norme{X - ZR\Lambda}_F$ in general, but it is an improvement
%on $R$ alone, and both stages can be solved quite easily.



% full algorithm goes here
